Nonlinear Distortion Radiated from Large Arrays and Active Reconfigurable Intelligent Surfaces

Extremely large aperture arrays (ELAAs) and reconfigurable intelligent surfaces (RISs) are candidate enablers to realize connectivity goals for the sixth-generation (6G) wireless networks. For instance, ELAAs can provide orders-of-magnitude higher area throughput compared to what massive multiple-input multiple-output (MIMO) can deliver through spatial multiplexing, while RISs can improve the propagation conditions over wireless channels but a passively reflecting RIS must be large to be effective. Active RIS with amplifiers can deal with this issue. In this paper, we analyze the distortion generated by nonlinear amplifiers in both ELAAs and active RIS. We derive analytical expressions for the angular directions and depth of nonlinear distortion in both near-field and far-field channels. These insights are then used in a distortion-aware scheduling scheme that predicts the beamforming directions of the distortion and strategically allocates users in frequency to minimize its impact. Numerical results validate our theoretical analysis and compare distortion-aware and distortion-unaware scheduling methods, highlighting the benefits of accounting for nonlinearities. We conclude that nonlinearities can both create in-band and out-of-band distortion that is beamformed in entirely new directions and distances from the transmitter.

==> response_letter01/01-overview.tex <==
We would like to thank the reviewers for their insightful comments and suggestions as well as the editor for handling this paper. We have thoroughly revised our manuscript based on your feedback.
Below, we provide an overview of the major changes made to the paper:
\begin{enumerate}
    \item {\bf Model Extension:} We have expanded the 3rd order memoryless model to a memory polynomial model with an arbitrary polynomial order and memory length. This enhancement has led to modifications in Theorem 1, which now provides the directions of distortion for any order of nonlinear distortion. This change allows for a more comprehensive analysis and a broader application of the results.

    \item  {\bf New Section on Numerical Results:} We have added a new section in the numerical results to demonstrate how nonlinear distortion impacts the performance of the network. This section specifically considers the effects under linear precoders, namely Maximum Ratio Transmission (MRT) and Zero Forcing (ZF). This addition aims to provide a clearer understanding of the practical implications of our theoretical findings.
    
    \item \textit{\bf Enhanced Visual Representation:} To aid in the comprehension of our system model and theoretical analysis, we have included a new figure that better represents the adopted Cartesian coordinate system. This visual enhancement is intended to facilitate a better understanding of the foundational concepts discussed in the paper. 
    
\end{enumerate}

We believe these revisions have significantly strengthened the paper and addressed the concerns raised during the review process. We appreciate the opportunity to improve our work and thank you for your valuable guidance.
In the following,  we present our point-by-point responses to the comments and indicate how our manuscript has been revised. The modifications in the manuscript are marked in  {\blue{blue}}.

% The comments helped to improve the quality of our work. 
% Before presenting our responses in detail, we summarize the major changes in the revised manuscript as follows:
% \begin{enumerate}
% \item Guided by Reviewers 1 and  4, we have added ...
% more simulation results in Section VII-C for a $64$-QAM modulation scheme and low dimensional MIMO systems which are currently of high interest, especially for 5G smartphones. In addition, we draw the quantiles to quantiles (QQ) plot to analyse the distribution of the residual noise in the MP detectors as suggested by the Reviewer 1.  
% \item  Guided by Reviewers 1 and 2, we have revised ...
% % our classification of the MIMO detectors and mentioned the sphere decoder that approaches the ML performance. 
% \item  Guided by Reviewers 2 and  3, we have ... 
% % moved the definition of the detection problem to the end of the Section II and added more explanation regarding the ML detection. In addition, we have added numerical complexity values in the last column of Table II to give the reader an intuitive understanding of the complexity comparison of the detectors.
% \item Guided by all Reviewers we have improved the quality of the presentation by correcting the typographical and citation errors, revising the organization of the manuscript, specifying parameters needed for the proposed detectors, clarifying the derivation of some variables, and mentioning ...
% % the generation of the ill-conditioned channel.
% \end{enumerate}



% \vspace{0.2cm}

% \noindent Sincerely,

==> response_letter01/02-reviewer1.tex <==
% ----------------------------------------------------------------%
%                       Reviewer 1                                %
% ----------------------------------------------------------------%

\section*{\underline{Response to Reviewer's 1 Comments}}
\label{sRev1}
\vspace{0.5cm}
We would like to thank the reviewer for his/her detailed review of our work. We found all the comments very constructive and motivating for improving the quality of our paper. 
In the following, a step-by-step response to all these comments is given.
\vspace{0.5cm}


% ----------------------------------------------------------------%
%                       QUESTION 1                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[1.]{\bf Comment:} The motivations of adopting the three-order memoryless polynomial distortion model for the PAs should be better explained. Can the method be extended to the higher-order memory PAs?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} 
Thank you for your suggestion. Indeed, Theorem 1 can be extended to accommodate higher-order memory polynomial PAs. We have updated the non-linear model in our paper to include the memory polynomial model, allowing for an arbitrary order of nonlinearities. Consequently, Theorem 1 now yields the directions of distortion for any order of nonlinearity. Appendix A has been revised accordingly to reflect these changes. Below, we present all updates in detail.
 
Let the discrete baseband transfer function of the nonlinear amplifier with memory be modeled by\cite{Ermolova2009,Zhou2004}
\begin{align}\label{eq:memory_model}
    \mathcal{A}\left(x_m[n] \right) = \sum_{p=0}^P\sum_{l=0}^L \beta_{2p+1}[l]x_m[n-l]\left|x_m[n-l]\right|^{2p},
\end{align}
where $ \beta_{2p+1}[l]$ are the coefficients (or kernels) of the amplifier, $P$ is the non-linearity order and $L$ is the memory length. Notice that when $L=0$, then the PA's model in \eqref{eq:memory_model} becomes memoryless.

To determine the directions and range of the $p$-th order and the $l$-th memory tap for the non-linear distortion, we express the radiation pattern of the distortion in terms of the array factor, i.e.,
\begin{align} \label{eq:array_factor}
    {\tt AF}_{2p+1}^{(l)}(\varphi,\theta,r) = \beta_{2p+1}[l] \sum_{m=1}^{M}a_m(\varphi,\theta,r)x_m[n-l]|x_m[n-l]|^{2p},
\end{align}
where $a_m(\cdot,\cdot,\cdot)$ is the line-of-sight channel between the $m$-th antenna element and a point $(\varphi,\theta,r)$, which is given by
\begin{align} 
    a_m(\varphi, \theta, r) &\approx e^{j\frac{2\pi}{\lambda}\tilde{\phi}_m(\varphi, \theta, r)},\label{eq:fresnel_apprx}
\end{align}
where the first-order Taylor approximation of channel's phase is given by
\begin{align}
    \begin{split}
    \tilde{\phi}_m(\varphi,\theta,r) = 
    k_z(m)\sin\theta  + k_y(m)\sin\varphi \cos\theta+
    \left( k^2_y(m) + k^2_z(m) \right)\frac{1}{2r}.
    \end{split}\label{eq:phase_apprx}
\end{align}

Furthermore, the transmitted symbol before amplification at the $m$-th antenna element can be expressed in the exponential form as 
\begin{align} \label{elaa:bb_tx_signal}
 x_m[n] = \sum_{k=1}^K \alpha_{mk}e^{-j\frac{2\pi}{\lambda}\phi_{m}\left(\varphi_k,\theta_k,r_k \right)} s_k[n],
\end{align}
where $\alpha_{mk} \in \mathbb{R}^{+}$ and $\phi_{m}\left(\varphi_k,\theta_k,r_k \right)\in \mathbb{R}$ are the modulus and phase of the precoder, respectively, while $s_k[n]$ is the time-domain symbol intended for the $k$-th user. 
\begin{Remark}
    It is important to note that expression \eqref{elaa:bb_tx_signal} represents a general form of a linear precoder. Therefore, the following proof can be applied to any precoder of this form. Specifically, in the case of maximum-ratio tranmission (MRT) or zero-forcing (ZF) precoders considered in this paper, we demonstrate in Reviewer 1, Question 3 that  $\alpha_{mk} = 1$. However, to maintain simplicity and consistency, we present the proof for the special cases of MRT and ZF in the updated paper.
\end{Remark}
Now, by substituting (\ref{elaa:bb_tx_signal})  into $x_m[n-l]|x_m[n-l]|^{2p}$, we get the expression
\begin{align}
\begin{split}\label{eq:nonlinear-factor}
    x_m[n-l]\left|x_m[n-l]\right|^{2p} = \left( x_m[n-l]\right) ^{p+1}\left( x_m^{\ast}[n-l]\right)^{p}\\
    = \sum_{k_0=1}^{K}\sum_{k_2=1}^{K}\cdots \sum_{k_{2p}=1}^{K}  \alpha_{mk_0}s_{k_0}[n-l] \alpha_{mk_2}s_{k_2}[n-l] \dots \alpha_{mk_{2p}} s_{k_{2p}}[n-l]\\
    \times e^{-j\frac{2\pi}{\lambda} \sum_{i=0}^p \phi_{m}\left(\varphi_{k_{2i}},\theta_{k_{2i}},r_{k_{2i}} \right)   }\\
    \times \sum_{k_{1}=1}^{K}\sum_{k_{3}=1}^{K}\cdots \sum_{k_{2p-1}=1}^{K}  \alpha_{mk_1}s^{\ast}_{k_1}[n-l] \alpha_{mk_3}s^{\ast}_{k_3}[n-l] \dots \alpha_{mk_{2p-1}} s^{\ast}_{k_{2p-1}}[n-l]\\
    \times e^{j\frac{2\pi}{\lambda} \sum_{i=1}^{p} \phi_{m}\left(\varphi_{k_{2i-1}},\theta_{k_{2i-1}},r_{k_{2i-1}} \right) }\\
    = \sum_{k_{0}=1}^{K}\sum_{k_{1}=1}^{K}\cdots \sum_{k_{2p}=1}^{K}
     \underbrace{s_{k_{0}}[n-l]s^{\ast}_{k_{1}}[n-l]\cdots s^{\ast}_{k_{2p-1}}[n-l] s_{k_{2p}}[n-l]}_{\triangleq 
 s_{{\boldsymbol k}}[n-l]}\\
    \times g_m({\boldsymbol k}) e^{-j\frac{2\pi}{\lambda}  \sum_{i=0}^{2p} (-1)^{i} \phi_{m}\left(\varphi_{k_{i}},\theta_{k_{i}},r_{k_{i}} \right) },
 \end{split}
\end{align}
where ${\boldsymbol k} \triangleq \left( k_{0},k_{1},\dots, k_{2p}\right) $ and $g_m({\boldsymbol k}) \triangleq \alpha_{mk_0}\alpha_{mk_1}\cdots \alpha_{mk_{2p}}\ge 0$. Additionally, for notational convenience, we define the phase of the $p$-th order of nonlinear distortion in \eqref{eq:nonlinear-factor} as
\begin{align}
    \tilde{\phi}_m(\varphi_{\boldsymbol k},\theta_{\boldsymbol k},r_{\boldsymbol k}) \triangleq \sum_{i=0}^{2p} (-1)^{i} \phi_{m}\left(\varphi_{k_{i}},\theta_{k_{i}},r_{k_{i}} \right)
\end{align}
and it can be re-written in the form of expression \eqref{eq:phase_apprx} as follows:
\begin{align}
    \begin{split}\label{eq:nonlinear-phase}
     \tilde{\phi}_m(\varphi_{\boldsymbol k},\theta_{\boldsymbol k},r_{\boldsymbol k})
        = k_z(m)\underbrace{\sum_{i=0}^{2p} (-1)^{i} \sin\theta_{k_i}}_{\triangleq \sin\theta_{\boldsymbol k}}+k_y(m)\underbrace{\sum_{i=0}^{2p} (-1)^{i} \sin\varphi_{k_i}\cos\theta_{k_i}}_{\triangleq \sin\varphi_{\boldsymbol k}\cos\theta_{\boldsymbol k}}\\
        -\frac{k^2_z(m)+k^2_y(m)}{2} \underbrace{\sum_{i=0}^{2p} (-1)^{i} \frac{1}{r_{k_i}}}_{\triangleq \frac{1}{r_{\boldsymbol k}}}.
    \end{split}
\end{align}

Then by substituting \eqref{eq:nonlinear-factor} into \eqref{eq:array_factor}, the array factor of the $p$-th order and the $l$-th memory tap becomes
\begin{align}
    \begin{split}\label{eq:array_factor_3}
    {\tt AF}_{2p+1}^{(l)}(\varphi,\theta,r)  \approx  \beta_{2p+1}[l] \sum_{k_{0}=1}^{K}\sum_{k_{1}=1}^{K}\cdots \sum_{k_{2p}=1}^{K}   
    s_{\boldsymbol k}[n-l]\\
    \times \underbrace{  \sum_{m=1}^{M} g_m({\boldsymbol k}) e^{-j\frac{2\pi}{\lambda} \left(  \tilde{\phi}_m(\varphi,\theta,r) - \tilde{\phi}_m(\varphi_{\boldsymbol k},\theta_{\boldsymbol k},r_{\boldsymbol k})    \right) }}_{\triangleq  
 {\tt AF}_{\boldsymbol k}(\varphi,\theta,r)},
 \end{split}
\end{align}
where the effective azimuth $\varphi_{\boldsymbol k}$, elevation $\theta_{\boldsymbol k}$ and range $r_{\boldsymbol k}$ of the nonlinear distortion are given by the following expressions after solving their corresponding equations as defined in expression \eqref{eq:nonlinear-phase}:
\begin{align}
    \theta_{\boldsymbol k} &= \arcsin\left( \sum_{i=0}^{2p} (-1)^{i} \sin\theta_{k_i}   \right) ,\\
    \varphi_{\boldsymbol k}  &= \arcsin\left( \frac{1}{\cos\theta_{\boldsymbol k}} \sum_{i=0}^{2p} (-1)^{i} \sin\varphi_{k_i}\cos\theta_{k_i} \right), \\
    r_{\boldsymbol k} &= \left( \sum_{i=0}^{2p} (-1)^{i} \frac{1}{r_{k_i}} \right)^{-1}.
\end{align}

Now, the amplitude of the term ${\tt AF}_{\boldsymbol k}(\varphi,\theta,r)$ can be upper bounded using the generalized triangle inequality as
\begin{align}
    |{\tt AF}_{\boldsymbol k}(\varphi,\theta,r)| &\le \sum_{m=1}^{M}\left| g_m({\boldsymbol k}) e^{-j\frac{2\pi}{\lambda} \left(  \tilde{\phi}_m(\varphi,\theta,r) - \tilde{\phi}_m(\varphi_{\boldsymbol k},\theta_{\boldsymbol k},r_{\boldsymbol k})\right)}\right|\label{eq:triangle-inequality}\\
    & =  \sum_{m=1}^{M} \left| g_m({\boldsymbol k}) \right|\label{eq:sum-of-abs}\\
    & = \sum_{m=1}^{M} g_m({\boldsymbol k}),\label{eq:sum}
\end{align}
where the last equation follows from the fact that $g_m({\boldsymbol k})\ge 0$. Therefore, the equality in \eqref{eq:triangle-inequality}  holds if and only if the channel vector equals that of the effective precoder, i.e.,
\begin{align}
    \tilde{\phi}_m(\varphi,\theta,r) =  \tilde{\phi}_m(\varphi_{\boldsymbol k},\theta_{\boldsymbol k},r_{\boldsymbol k})
\end{align}

Therefore, the term $|{\tt AF}_{\boldsymbol k}(\varphi, \theta,r)|$ is maximized at the points where $(\varphi, \theta,r) = (\varphi_{\boldsymbol k}, \theta_{\boldsymbol k},r_{\boldsymbol k})$ for $k_i = 1,2,...,K$ and $i=0,1,...,2p$.

\end{itemize}





% ----------------------------------------------------------------%
%                       QUESTION 2                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[2.]{\bf Comment:} The authors are suggested to provide a figure for better representing the adopted Cartesian coordinate system, which is the basis of your derivations and conclusions.
\end{itemize}
\end{minipage}}


\begin{itemize}
\item[]{\bf Response:} Thank you for your suggestion. We have enhanced the revised paper with the Fig. \ref{figure_geometric_setup} below.

\begin{figure}[t!]
	\centering 
	\begin{overpic}[width=.5\columnwidth,tics=10]{figures/geometric_setup.pdf}
		\put(54,1){\footnotesize $x$}
		\put(60,39){\footnotesize $y$}
		\put(9.5,57){\footnotesize $z$}
		\put(26.5,10){\footnotesize  $\varphi$}
		\put(40,17){\footnotesize  $\theta$}
		\put(5,11){\footnotesize  $1$}
		\put(1.5,41){\footnotesize  $N_{y}$}
		\put(12.7,54){\footnotesize  $1$}
		\put(46,74){\footnotesize  $N_{z}$}
		\put(80,31){\footnotesize  LoS path}
		%\put(80,27){\footnotesize  component}
\end{overpic} 
	\caption{The 3D geometry of an RIS consisting of $M_{y}$ elements per row and $M_{z}$ elements per column.}\vspace{-0.3cm}
	\label{figure_geometric_setup}  
\end{figure}

\end{itemize}



% ----------------------------------------------------------------%
%                       QUESTION 3                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[3.]{\bf Comment:} The reviewer is skeptical of the sentence “since the channel is line-of-sight (LoS), its frequency response is constant over frequency” above the Eq. (8). The authors should verify this conclusion and explain it more explicitly.
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} Thank you for raising this issue. Please note that the sentence, {\bf ``since the channel is line-of-sight (LoS), its frequency response is constant over frequency''}, was included in the original version of the paper to justify the expression \eqref{eq:ofdm_per_antenna} which is the basis for proving Theorem 1. In the updated version, we have removed this sentence to avoid confusion and have instead provided an analytical system model in Section II. Below, we present all updates in detail.

The {\bf line-of-sight} spherical wave channel model in the near-field region between the base station and user $k$ at the $\nu$-th subcarrier can be presented as\cite{Sherman1962,Symeon2023,Dai2022}
\begin{align}\label{eq:ofdm_channel_user}
    \hat\vech_k[\nu] = g_k\veca(\varphi_k,\theta_k,r_k) e^{-j2\pi \tau_k \nu},
\end{align}
where $\veca(\cdot)\in \mathbb{C}^{M\times 1}$ is the near-field steering vector, $g_k$  and $\tau_k$ are the is the complex path gain and delay of the signal from the first antenna at the base station to user $k$, respectively.
On this basis, the MIMO channel matrix $\hat{\matH}_\nu\in \mathbb{C}^{M\times K}$ can be expressed as
\begin{align}
       \hat{\matH}_\nu =  \underbrace{\left[ {\veca}_{1}\ {\veca}_{2}\ \dots\ {\veca}_{K}\right]}_{\triangleq \matA}\matF_\nu .
\end{align}
where ${\veca}_{k} \triangleq \veca(\varphi_k,\theta_k,r_k)$ is the channel (steering) vector between the base station and $k$-th user, given by
\begin{align}
       {\veca}_{k} =  \left[1\ e^{j\frac{2\pi}{\lambda} \phi_0(\varphi_k,\theta_k,r_k)}\ \dots \  e^{j\frac{2\pi}{\lambda} \phi_{M-1}(\varphi_k,\theta_k,r_k)}\right]^T
\end{align}
and the $K\times K$ matrix $\matF_\nu$ is a diagonal matrix with its $k$-th diagonal entry being $g_ke^{-j2\pi \tau_{k} \nu}$.
The precoders that are considered in this work are MRT and the ZF, respectively, given by the following expressions: 
\begin{align}
    \mathcal{P}\left(\hat{\matH}_\nu\right) &=  {\matA^{\ast}}\matF_\nu^{\ast},\label{eq:mrt}\\
    \mathcal{P}\left(\hat{\matH}_\nu\right) &=  \matA^{\ast}\underbrace{\left( \matF_\nu \matA^T \matA^{\ast} \right)^{-1}}_{\triangleq \matB_{\nu}},\label{eq:zf}
\end{align}
where the matrix $\matB_{\nu}\in \mathbb{C}^{K\times K}$ is defined for notational convenient. Notice that the expressions \eqref{eq:mrt} and \eqref{eq:zf} are valid when the $K$ co-scheduled users are assigned the same subcarriers. 
Then, by employing the MRT precoder, the OFDM time-domain vector $\vecx_n$ before amplification at time sample $n$ $(n=0,\ldots, N-1)$ is obtained from the data symbols as
\begin{align}
\vecx_n &= \frac{1}{\sqrt{N}}\sum_{\nu\in \mathcal{S}}{\matA^{\ast}\matF^{\ast}_\nu}\vecs_\nu e^{j\frac{2\pi}{N}n\nu}\notag \\
        &= \matA^{\ast}\vecs_n,\label{eq:ofdm_symbol}
\end{align}
 where $\vecs_n \triangleq (1/\sqrt{N}) \sum_{\nu\in \mathcal{S}}{\matF^{\ast}_\nu}\vecs_\nu e^{j\frac{2\pi}{N}n\nu}$. It is important to note that when using the ZF precoder, we obtain a similar expression to \eqref{eq:ofdm_symbol} by substituting $\matF_{\nu}$ with $\matB_{\nu}$. Thus, from now on, we will focus on MRT.
 Let $e^{j\phi_m\left(\varphi_k,\theta_k,r_k \right)}$ represent the $(m,k)$-th entry of $\matA^{\ast}$, where $\phi_{m}(\cdot,\cdot,\cdot) \in \mathbb{R}$ denotes the phase of the precoder at the $(m,k)$-th entry.
Then, from (\ref{eq:ofdm_symbol}), the transmitted symbol before amplification at the $m$-th antenna element can be expressed as 
\begin{align} \label{eq:ofdm_per_antenna}
 x_m[n] = \sum_{k=1}^K e^{-j\frac{2\pi}{\lambda}\phi_{m}\left(\varphi_k,\theta_k,r_k \right)}s_{k}[n],
\end{align}
where $s_k[n]$ is the $k$-th entry of the vector $\vecs_n$.
The expression \eqref{eq:ofdm_per_antenna} is equivalent to that in \eqref{elaa:bb_tx_signal}, which is the basis for proving Theorem 1. 

Recall that in the expression \eqref{eq:ofdm_per_antenna}, we assume a multi-user scenario where all users allocate the same subcarriers. This assumption is made solely to simplify the proof of Theorem 1. In the general case, where different users are allocated to different pieces of bandwidth, the expression \eqref{eq:ofdm_per_antenna} becomes
\begin{align} \label{eq:general_ofdm}
 x_m[n] = \sum_{\nu\in \mathcal{S}}\sum_{k\in \mathcal{K}_\nu} e^{-j\frac{2\pi}{\lambda}\phi_{m}\left(\varphi_k,\theta_k,r_k \right)}
 s_{k}[n,\nu],
\end{align}
where $\mathcal{K}_\nu$ denotes the index set of users that are served on subcarrier $\nu$ and 
\begin{align}
    s_{k}[n,\nu] \triangleq g_ke^{-j2\pi \tau_k \nu}e^{-j\frac{2\pi}{N} n \nu}s_k[\nu],
\end{align}
where $s_k[\nu]$ is the $k$-th entry of the vector $\vecs_\nu$.
One can easily generalize the proof using the set notation that you present in \eqref{eq:general_ofdm}. It can be shown that the directions of distortion in Theorem 1 still hold even in this case that different users allocate use different bandwidth, although they will exhibit different power levels.%\cite[Theorem 4]{mollen_spatial}. 


\end{itemize}


% ----------------------------------------------------------------%
%                       QUESTION 4                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[4.]{\bf Comment:} In Section IV, the authors “consider an active RIS with N reconfigurable elements”. However, the RIS beamforming matrix in Eq. (25) is of the dimension M by M. Please explain it.
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} Thank you for noticing this typo. We have revised the notation for the number of RIS elements to $M$ and ensured it is consistent throughout the paper.
\end{itemize}



% ----------------------------------------------------------------%
%                       QUESTION 5                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[5.]{\bf Comment:} What are the differences and associations between $\phi_{s}$ and $\phi_{k}$?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} The angle $\varphi_k$ corresponds to the azimuth direction where the RIS observes the user $k$ for $k=1,\ldots,K$, while the angle $\varphi_s$ corresponds to the azimuth shift of the impinging signal from the RIS. 
For example, when the impinging signal from the user $k$ arrives from the azimuth angle $\varphi_k$, then the signal is reflected towards the azimuth angle $\varphi_s-\varphi_k$.
\end{itemize}



% ----------------------------------------------------------------%
%                       QUESTION 6                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[6.]{\bf Comment:} The derivation seems to rely on the assumption of identical $g_{mpqv}$. Whether the derivation and conclusion still hold when $g_{mpqv}$ differs with different values of $m$, $p$, $q$ and $v$?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} The conclusion holds in more general cases.
Please notice that in the revised version, the variable $g_{mpqv}$ has been changed to $g_m({\boldsymbol k})$ to facilitate any order of nonlinear distortion, where the vector ${\boldsymbol k}$ represents now the values of $p$, $q$ and $v$ from the previous version. 

As demonstrated in equations \eqref{eq:triangle-inequality}-\eqref{eq:sum} in response to your first comment, we have revisited the proof to ensure that it remains valid for any value of $g_m({\boldsymbol k})$, thus addressing your concern.
\end{itemize}



% ----------------------------------------------------------------%
%                       QUESTION 7                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[7.]{\bf Comment:} If the active RIS is replaced with full-duplex relay, can the proposed scheme achieve better performance?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} Please notice that the primary focus of our paper is to analyze the nonlinear distortion in ELAA and active RIS. While the performance comparison with full-duplex relays is an interesting and relevant topic, it falls outside the scope of our current study. Our work aims to contribute to understanding nonlinear effects in RIS specifically. 

A performance comparison with full-duplex relays would boil down to a case study where analytical and numerical comparisons are made for different typical propagation scenarios and assumptions.
We acknowledge the importance of this comparison and in the Section I, we suggest that readers refer to existing literature such as \cite{BJornson2020, DiRenzo2020, Ding2024} that specifically addresses the performance of RIS versus full-duplex relays. We appreciate your suggestion, and it might serve as a valuable direction for future research.
\end{itemize}



% ----------------------------------------------------------------%
%                       QUESTION 8                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[8.]{\bf Comment:} The authors should present more results to illustrate how the distortion affect the ultimate performance (e.g., throughput).
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} Thank you for your suggestion. To demonstrate the performance of the network (i.e., throughput) as well as the radiation patterns of the desired (linear) signal and nonlinear distortion, we decompose the output of a PA, which is modeled by the memory polynomial in \eqref{eq:memory_model}, to its statistical equivalent linear form as\cite{Ermolova2009}:
\begin{align}\label{eq:bussgang}
    y_m[n] = \underbrace{h_m[n]\star x_m[n]}_{\triangleq u_m[n]} + d_m[n],
\end{align}
where the linear term $u_m[n]$ represents the desired signal while $d_m[n]$ represents the nonlinear distortion, which is uncorrelated to the input signal $x_m[n]$. Moreover, the term $h_m[n]$ is given by \cite{Ermolova2009}
\begin{align}
    h_m[n] = \sum_{q=0}^Q (q+1)!P_{\tt in,m}^q\beta_{2q+1}[n],
\end{align}
where $P_{\tt in,m} \triangleq [C_{\bf{xx}}[0]]_{m,m} $ is the input signal power to the $m$-th antenna element.
The frequency-domain transmit signal in \eqref{eq:bussgang} at the $\nu$-th subcarrier is given by
\begin{align}\label{eq:linear-equivalent-frequency}
    \hat{y}_m[\nu] = \hat{h}_m[\nu] \hat{x}_m[\nu] + \hat{d}_m[\nu],\hspace{4mm} m=1,2,...,M,
\end{align}
where the variables $\hat{y}_m[\nu]$, $\hat{h}_m[\nu]$, $\hat{x}_m[\nu]$  and $\hat{d}_m[\nu]$ denote the discrete Fourier transform of $y_m[n]$, $h_m[n]$, $x_m[n]$ and $d_m[n]$, respectively. 
Furthermore, the expression \eqref{eq:linear-equivalent-frequency} can be re-written in a vector form as
\begin{align}
    \hat{\vecy}_{\nu} = \hat\matG_{\nu} \hat{\vecx}_{\nu} + \hat{\vecd}_{\nu},
\end{align}
where the $m$-th element of the $M\times 1$ vectors $\hat{\vecy}_{\nu}$, $\hat{\vecx}_{\nu}$ and $\hat{\vecd}_{\nu}$ correspond to the variables $\hat{y}_m[\nu]$, $\hat{x}_m[\nu]$ and $\hat{d}_m[\nu]$, respectively. Furthermore, the $M\times M$ matrix $\hat\matG_{\nu}$ is diagonal, where its $m$-th diagonal element is the variable $\hat{h}_m[\nu]$. Now, let $\hat\vech_k[\nu]$ be the $M\times 1$ LoS channel from the base station to user $k$ as defined in \eqref{eq:ofdm_channel_user}.
Then, the received signal $r_{k}[\nu]$ on the $\nu$-th subcarrier for the $k$-th user is given by
\begin{align}
    r_{k}[\nu] &= \hat\vech_k^T[\nu]\hat\matG_{\nu} \matP\matF^{\ast}_{\nu}\vecs_{\nu} + \hat\vech_k^T[\nu]\hat{\vecd}_{\nu} + n\\
     &= \underbrace{\hat\vech_k^T[\nu] \hat\matG_{\nu} \matP_{k} s_k[\nu]e^{j2\pi\tau_k\nu}}_{\text{signal}} + \underbrace{\sum_{i\neq k}\hat\vech_k^T[\nu] \hat\matG_{\nu} \matP_{i}  s_i[\nu]e^{j2\pi\tau_i\nu}}_{\text{interference}} + \underbrace{\hat\vech_k^T[\nu]\hat{\vecd}_{\nu}}_{\text{distortion}} + \underbrace{n}_{\text{noise}},
\end{align}
where $\matP_{k}$ denotes the $k$-th column of the precoder $\matP$ defined in the expressions \eqref{eq:mrt} and \eqref{eq:zf}. Therefore, the signal-to-interference-noise-and-distortion ratio (SINDR) is given by
\begin{align}
    \gamma_{k}[\nu]=\frac{|\veca_k^T \hat\matG_\nu \matP_{k}|^2}{\sum_{i\neq k}|\veca_k^T \hat\matG_\nu \matP_{i}|^2+\veca_k^T\matS_{\tt dd}[\nu] \veca_k^{\ast}+\sigma_n^2},
\end{align}
where $\matS_{\tt dd}[\nu]$ is the power spectral density (PSD) of the distortion and is given by the Fourier transform of the distortion's covariance matrix $\matC_{\tt dd}[\tau] \triangleq\mathbb{E}\left\{{\vecd}_n{\vecd}_{n-\tau}^H\right\}$. The matrix $\matS_{\tt dd}[\nu]$ can be calculated analytically by using the fact that the distortion is uncorrelated to the input signal. That is,  
\begin{align}
    \matS_{\tt dd}[\nu] = \matS_{\tt yy}[\nu] - \widehat\matG_\nu \matS_{\tt xx}[\nu] \hat\matG_\nu^{\ast},
\end{align}
where the PSD of the pre-amplified signal $\vecx$ is $\matS_{\tt xx}[\nu] = \matP\matP^H$, while the PSD of the output signal $\matS_{\tt yy}[\nu]$ is derived analytically in \cite[Eqs.~(48)]{Zhou2004} for the PA model in \eqref{eq:memory_model}. 
Then, we can obtain the achievable sum rates of the maximum-ratio and zero-forcing using the following expression:
\begin{align}
    R_{\tt sum} = \frac{1}{S}\sum_{k=1}^K\sum_{\nu\in S}\log_2\left( 1 + \gamma_{k}[\nu] \right).
\end{align}
\end{itemize}


\begin{figure*}
\begin{multicols}{2}
  \includegraphics[width=\linewidth]{figures/achievable_rates_4x4.eps}\par\caption{Sum rate as a function of SNR for different levels of EVM with $M=16$ antennas.}\label{fig:sum_rate_16}
    \includegraphics[width=\linewidth]{figures/achievable_rates_10x10.eps}\par\caption{Sum rate as a function of SNR for different levels of EVM with $M=100$ antennas.}\label{fig:sum_rate_100}
\end{multicols}
\end{figure*}

The next paragraph has been added to the Numerical results:

\textcolor{blue}{
We present the numerical results to demonstrate the impact of nonlinear distortion on the sum rate as a function of the signal-to-noise ratio (SNR). The performance is evaluated using MRT and ZF precoders for two different configurations of the number of antennas.
Specifically, Fig. \ref{fig:sum_rate_16} illustrates the sum rate as a function of the SNR for different levels of EVM (i.e., $0$ and $0.3$). 
% In this example, the system is equipped with $M=16$ antennas. 
When the nonlinear distortion is zero (i.e., EVM $= 0$), the sum rate increases linearly with the SNR for ZF,  as it effectively cancels inter-user interference. However, when introducing an EVM of $0.3$ results, there is a noticeable degradation in the sum rate at a high-SNR regime due to the presence of nonlinear distortion, which cannot be mitigated by ZF.
Conversely, MRT precoding does not mitigate inter-user interference, which dominates the distortion. Thus, the performance degradation is negligible in the presence of nonlinear distortion.
Fig. \ref{fig:sum_rate_100} shows the sum rate as a function of SNR with a system equipped with $M=100$ antennas. Notice that the introduction of nonlinear distortion results in a significant reduction in the sum rate, especially at higher SNR values. With $M=100$ antennas, the performance degradation due to distortion is more pronounced than in the $M=16$ case, demonstrating that the higher the number of antennas, the greater the received power of distortion at the UEs.
These results clearly demonstrate the impact of EVM on system performance, emphasizing the importance of minimizing EVM to achieve higher sum rates, particularly in scenarios with a larger number of antennas and higher SNR values. The analysis shows that while ZF precoding can handle inter-user interference effectively under ideal conditions, its performance degrades significantly in the presence of nonlinear distortion. On the other hand, MRT precoding shows resilience to nonlinear distortion, but its overall performance is limited by inter-user interference.
}
\begin{comment}
    To demonstrate this claim, let $h_{km}(\tau)$ denote the channel's impulse response from the $m$-th antenna element to user $k$. In the frequency domain, its transfer function is
\begin{align}\label{eq:channel-tranfer-function}
    \hat{h}_{km}(f) = \int_{-\infty}^{\infty} h_{km}(\tau) e^{-j2\pi \tau f}d\tau.
\end{align}
In the special case where the channel is LoS, its  transfer function becomes
\begin{align*}
    \hat{h}_{km}(f) = h_{km}(\tau_{km}) e^{-j2\pi \tau_{km} f},
\end{align*}
where $\tau_{km}$ is the delay of the signal from the reference antenna to user $k$ associated with the $m$-th antenna element. Note that the distinction in the time of arrival of the signal among the antenna elements arises from the nature of the near-field channel. Then, the channel response is given by
\begin{align}
   \hat{h}_{km}(f) =  e^{-j2\pi \left( \tau_{km} f - \phi_m(\varphi_k,\theta_k,r_k)/\lambda \right)}.
\end{align}
We operate under the narrowband assumption, which implies that the signal’s limited bandwidth leads to poor time delay resolution. This limitation makes it challenging for the base station to distinguish between users with closely spaced delays. However, due to the spherical waveform in the near-field, the received signal from users will arrive at the antennas at various time delays, denoted as $\tau_m$. Consequently, it is assumed that the signals from all users arrive simultaneously at the $m$-th antenna, approximated as $\tau_{km}\approx\tau_m$.
\end{comment}

==> response_letter01/03-reviewer2.tex <==
% ----------------------------------------------------------------%
%                       Reviewer 2                                %
% ----------------------------------------------------------------%

\section*{\underline{Response to Reviewer's 2 Comments}}
\vspace{0.5cm}
We thank the Reviewer for raising a number of important points in his/her review. In the
following, a step-by-step response to all these comments is given.
\vspace{0.5cm}

% ----------------------------------------------------------------%
%                       QUESTION 1                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[1.]{\bf Comment:} The element of a RIS usually called "unit cell" to distinguish RISs from antenna arrays.
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} In the revised manuscript, we have replaced the term ``element" for the RIS with ``unit cell" or  ``cell" as you suggested.
\end{itemize}


% ----------------------------------------------------------------%
%                       QUESTION 2                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[2.]{\bf Comment:} For an active RIS, what's its difference to a transmitting antenna array (using a same amplifier) when analyze the nonlinear distortion?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} 
When analyzing nonlinear distortion, the primary difference between an active RIS and a transmitting antenna array, even though their behavioral analysis is the same, lies in the source and nature of the parameters that influence the distortion.

For a transmitting antenna array, the distortion's characteristics are influenced by the selection of the digital precoder, which determines its spatial directions, as shown in Theorem 1.

On the other hand, for an active RIS, the distortion characteristics are primarily determined by the directions of the impinging signal and the phase shifts applied by the RIS elements. The RIS reflects incoming signals by adjusting the phase of each unit cell, and these phase adjustments, along with the angle of incidence, influence the nonlinear behavior of the system, as shown in Corollary 5.


\end{itemize}



% ----------------------------------------------------------------%
%                       QUESTION 3                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[3.]{\bf Comment:} Is the results tenable for other systems besides OFDM systems?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} The analysis in the paper is independent of the OFDM system. 
 As presented in Theorem 1, the non-linear distortion analysis is mathematically developed based on the structure of the precoding matrix. 
 % used to beamform the signal in multiple directions. 
 Through Theorem 1, we gain the primary novel insight of this paper, i.e., the distortion is beamformed in the same direction but spreads to different distances,
 % than those of the users, 
 according to the given analysis. Therefore, this analysis applies not only to OFDM systems but can also be generalized to other systems.
\end{itemize}


% ----------------------------------------------------------------%
%                       QUESTION 4                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[4.]{\bf Comment:} References should be cited in order.
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} We have rechecked the order of the references to ensure they are properly arranged. For example, we reordered references [10] and [11] to align with the chronological order of their publication years.
\end{itemize}

==> response_letter01/04-reviewer3.tex <==
% ----------------------------------------------------------------%
%                       Reviewer 3                                %
% ----------------------------------------------------------------%

\section*{\underline{Response to Reviewer's 3 Comments}}
\vspace{0.5cm}
We thank the Reviewer for raising a number of important points in his/her review. In the
following, a step-by-step response to all these comments is given.
\vspace{0.5cm}

% ----------------------------------------------------------------%
%                       QUESTION 1                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[1.]{\bf Comment:} What is the guiding significance of studying nonlinear distortion to the actual transmission system? How can we eliminate or alleviate the influence caused by nonlinearity?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} Thank you for your insightful question. Studying nonlinear distortion is crucial for understanding and improving the performance of actual transmission systems. As shown in \textbf{Reviewer's 1, Question 8}, nonlinear distortion can significantly reduce system performance.

The community is used to designing hardware components with low distortion values in practical systems to mitigate distortion at the design level. However, that might no longer be viable when considering very large arrays (as in this paper). 
By thoroughly analyzing the sources and impacts of nonlinear distortion, we can develop strategies to mitigate these effects also at the signal processing level, thereby enhancing the reliability and performance of communication systems.

For example, we can exploit the theory presented in this paper to predict the beamforming directions of the distortion created by the nonlinear amplifiers. This could potentially be used to schedule users in frequency in such a way that the influence of the distortion is minimized. Specifically, if a large portion of the spectrum is beamformed towards a single user, another user with a similar channel should not be scheduled to use subcarriers close to that user. With a deep understanding of the distortion structure, one can potentially also modify the beamforming methods to control where the non-linear distortion ends up.

We have updated Section I based on the aforementioned discussion of the revised manuscript as follows:


\blue{``We derive a theorem that analytically characterizes the angular directions and depth of nonlinear distortion in the near-field region. This theory can help develop strategies to mitigate these effects at the signal processing level, enhancing communication system reliability and performance. For example, the predicting the beamforming directions of the distortion in Theorem 1, it could be used to schedule users in frequency and space to minimize distortion influence."}


\end{itemize}


% ----------------------------------------------------------------%
%                       QUESTION 2                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[2.]{\bf Comment:} In section IV,“We now consider an active RIS with $N$ reconfigurable elements ...”, should $N$ be replaced by $M$?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} 
Thank you for identifying this typo. We have revised the notation for the number of RIS elements to $M$ and ensured it is consistent throughout the paper.
\end{itemize}



% ----------------------------------------------------------------%
%                       QUESTION 3                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[3.]{\bf Comment:} In section V, it is suggested to supplement the test results in the actual scene and compare them with simulation results.
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} In this paper, we focus on establishing the fundamentals of non-linear distortion in near-field communication scenarios from the theoretical perspective. Evaluating and validating the theoretical analysis in real-world implementations requires a huge prototyping effort, which we consider a valuable direction for future work. We appreciate the reviewer for pointing this out and have added the following discussion in Section I of the revised manuscript 


\blue{``In this paper, we analyze the distortion either transmitted by an ELAA or created by an active RIS that reflects multiple signals from a theoretical perspective in this paper."}

\end{itemize}


% ----------------------------------------------------------------%
%                       QUESTION 4                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[4.]{\bf Comment:} In Fig.~3 - Fig.~6, the PSD of the expected signal is about three orders of magnitude after considering distortion. Is it reasonable?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} Yes, please notice that in these plots we assume that the level of EVM is 3\% which means that the power nonlinear distortion should be 3\% of the total power.
\end{itemize}


% ----------------------------------------------------------------%
%                       QUESTION 5                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[5.]{\bf Comment:} In Fig.~3 - Fig.~6, it seems that the unit of PSD is not marked.
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} Thank you for your observation.
The correct unit for PSD should be dBm/Hz. We have updated the manuscript to include the unit for clarity.
\end{itemize}

==> response_letter01/05-reviewer4.tex <==
% ----------------------------------------------------------------%
%                       Reviewer 4                                %
% ----------------------------------------------------------------%

\section*{\underline{Response to Reviewer's 4 Comments}}
\vspace{0.5cm}
We would like to thank the Reviewer for providing such a stimulating and detailed review
report. In the following, a step-by-step response to all these comments is given.
\vspace{0.5cm}

% ----------------------------------------------------------------%
%                       QUESTION 1                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[1.]{\bf Comment:} The motivation is still not very clear. Specifically, why the authors study the nonlinear distortion of ELAA and active RIS together? What is the similarity and the difference of the nonlinear distortion of ELAA and active RIS?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} 
The main motivation for considering non-linear distortion in both ELAA and active RIS is their similar behavior regarding this effect so that our novel results obtained for ELAA can be applied to active RIS while only making minor modifications. The primary difference in the non-linear distortion behavior between the two cases is as follows: in ELAA, the non-linear distortion effect occurs when it sends the signal to the user equipment (UE), while in active RIS, the non-linear distortion occurs when amplifying and reflecting the user's signal to the base station (BS). To clarify this, in Section IV we have the following paragraph.

``...the behavioural analysis derived in Theorem 1 for an ELAA system, it can be also applied for an active RIS. However, in the latter case, the beamformed vector of each signal is not created in the baseband but comes from the channel from the users as well as we can modify the reflected angles using the RIS."


\end{itemize}


% ----------------------------------------------------------------%
%                       QUESTION 2                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[2.]{\bf Comment:} Why consider a third-order nonlinear distortion in the paper (the explanation in the footnote is not enough to demonstrate it)?  Does there exist another type of nonlinear distortion for ELAA and active RIS.
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} Thank you for this comment. In the revised manuscript we have extended the analysis to an arbitrary polynomial order of non-linear distortion. You can find the revised text in the manuscript, i.e. in System Model and Theorem 1, and in the response to \bf{Reviewer's 1, Question 1}.
\end{itemize}



% ----------------------------------------------------------------%
%                       QUESTION 3                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[3.]{\bf Comment:} The nonlinear distortion in tradition massive MIMO system has been studied. The considered setup with an ELAA is essentially a multiuser MIMO system. Thus, what is the difference of ELAA and the traditional massive MIMO system and what is the main contribution of the nonlinear distortion of the considered ELAA when compared with the nonlinear distortion in tradition massive MIMO system? We notice that ELAAs mean extremely large aperture arrays and the problem is that how to demonstrate the role of the so-called "extremely large" aperture arrays.
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} 
The main difference between the nonlinear distortion studied in this paper for Extremely Large Aperture Arrays (ELAA) and traditional massive MIMO is not merely about the number of antennas or the term "extremely large," which can be somewhat vague. The key distinction lies in our analysis of nonlinear distortion behavior radiated from a transmitter (either ELAA or active RIS) equipped with a planar array. This setup enables us to analyze the distortion in both the azimuth and elevation domains. In contrast, traditional massive MIMO studies typically focus on uniform linear arrays (ULAs), limiting distortion analysis to a single dimension (e.g., azimuth).

Furthermore, we examine the nonlinear distortion behavior in the context of near-field communications, which fundamentally differs from the traditional far-field communications in existing massive MIMO technology used in fifth-generation wireless systems. The previous studies that the reviewer refers to, and which are cited in the paper, analyze non-linear distortion in far-field scenarios.

Near-field communications arise because we employ a large aperture array, making the classical Fraunhofer distance boundary, which separates the far-field and near-field regions, very large. This boundary is inversely proportional to the aperture length of the array. As long as the distance between the array and the users is less than $2D^2/\lambda$, where $D$  is the aperture length of the array, the users will be in the near-field of the array.
When the arrays become larger and the wavelength shrinks in future systems, the Fraunhofer distance will become hundreds of meters, and most users will be in the near field.
In this scenario, new phenomena for beamforming the signal in the distance domain appear, making our study relevant. Previous works have considered the implications of this for distortionless communications. To the best of our knowledge, we are the first to study non-linear distortion under these new propagation conditions.
\end{itemize}


% ----------------------------------------------------------------%
%                       QUESTION 4                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[4.]{\bf Comment:} The current work only consider the channel response of the point source (user). The practical channel models with extend target (not a point of interest) user might be considered.
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} Please note that although the channel model presented in the system model represents the channel responses between the array and $K$ users, our simulation results extend the channel over the entire plane (azimuth, elevation) and depth (near-field). This is detailed in the last paragraph of Section V.B. Hence, we are analyzing the impact of the non-linear distortion in the way requested by the reviewer.

Additionally, Figs. 6 and 7 illustrate the radiation of distortion over all channel dimensions. This provides us with a 3D behavioral analysis of distortion in the entire space of the channel, including the azimuth, elevation, and depth domains.

\end{itemize}

==> response_letter02/01-overview02.tex <==
We would like to thank the reviewer for their insightful comments and suggestions, as well as the editor for their careful handling of our paper. We have thoroughly revised the manuscript in response to the feedback provided. Below, we outline the major changes made to the paper:

\begin{enumerate}

    \item  {\bf New Section on Numerical Results:} We have added a new section in the numerical results to demonstrate the utility of Theorem 1. Specifically, we present a scenario where the theorem is applied to predict the beamforming directions of non-linear distortion and to schedule users in both frequency and space, effectively minimizing the influence of distortion.
    

    
\end{enumerate}

We believe the revision has significantly strengthened the paper and addressed the concerns raised during the review process. We appreciate the opportunity to improve our work and thank you for your valuable guidance.
In the following,  we present our point-by-point responses to the comments and indicate how our manuscript has been revised. The modifications in the manuscript are marked in  {\blue{blue}}.



==> response_letter02/02-reviewer.tex <==
% ----------------------------------------------------------------%
%                       Reviewer 4                                %
% ----------------------------------------------------------------%

\section*{\underline{Response to Reviewer's 3 Comments}}
\vspace{0.5cm}
We thank the Reviewer 3 for raising a number of important points in his/her review. In the
following, a step-by-step response to all these comments is given.
\vspace{0.5cm}

% ----------------------------------------------------------------%
%                       QUESTION 1                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[1.]{\bf Comment:}  It is suggested to supplement more related research work on power amplifier nonlinearity, so that readers can better understand the motivation and contribution of the work;
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} Thank you for the suggestion. We have added the following paragraph to the introduction:

``\textcolor{blue}{Other studies \cite{ove, fredrik} highlight how nonlinear distortion critically affects MIMO systems and the trade-offs it imposes between system capacity and power efficiency. These insights reinforce the need to develop theoretical models that analyze the joint spatial and frequency behavior of such impairments, as done in this work, so the performance trade-offs can be rigorously optimized.}''



\end{itemize}


% ----------------------------------------------------------------%
%                       QUESTION 2                                %
% ----------------------------------------------------------------%


\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[2.]{\bf Comment:} In the contribution, the author mentioned ``For example, the predicting beamforming directions of the distortion in Theorem 1, it could be used to schedule users in frequency and space to minimize distortion influence." Can the author give a simulation example of user scheduling in the main body as an auxiliary illustration to highlight the contribution of this part?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} 
Thank you for your valuable suggestion. To address your comment, we explored a scenario designed to minimize the influence of distortion through user scheduling. Fig.~S1 illustrates the sum rate as a function of the signal-to-noise ratio (SNR) for two scheduling methods, i.e., distortion distortion-aware and distortion-unaware scheduling, using the following simulation setup:

We co-scheduled four users in a bandwidth of 128 subcarriers, with each user occupying 30 subcarriers chosen from a set of 12 users that are grouped into 4 clusters. Sub-band scheduling is employed, meaning that different users are allocated distinct parts of the bandwidth.
\begin{itemize}
    \item Users within a cluster are located very close to each other.
    \item The clusters themselves are significantly far apart.
\end{itemize}

To compare the performance, we evaluated the following scheduling methods:
\begin{enumerate}
    \item \textbf{Distortion-unaware scheduling (baseline method):}  
    In this method, users are scheduled randomly. This approach often results in co-scheduling users from the same cluster, exposing them to stronger out-of-band (OOB) emissions due to their physical proximity. These emissions exhibit the highest levels of power in the vicinity of the user (cf. Corollary 2), leading to increased distortion and reduced performance (see Figs. 4 and 5).

    \item \textbf{Distortion-aware scheduling (proposed method):}  
    In this method, we exploit Theorem 1  to predict the beamforming directions of distortion created by nonlinear amplifiers. This enables the minimization of OOB emissions by scheduling users in a way that avoids distortion. In this example, by preventing the co-scheduling of users from the same cluster, the method exploits the significant physical separation between clusters to reduce OOB distortion effects that would otherwise be beamformed toward users within the same cluster.
\end{enumerate}


\textbf{Key Observations:}
\begin{itemize}
    \item The proposed distortion-aware scheduling method achieves a \textbf{11.4\% gain} in sum rate for \textbf{EVM = 5\%} and a \textbf{15\% gain} for \textbf{EVM = 10\%} at high SNR (25~dB).
    \item That is, the performance gap widens as the EVM increases, showcasing the effectiveness of the proposed method in minimizing distortion influence in distortion-sensitive scenarios.
    \item At low SNR values, the difference between the two methods is negligible, as distortion effects are less significant in this regime.
\end{itemize}

These results validate the effectiveness of the proposed method in minimizing distortion influence and highlight its potential for improving system performance under hardware non-linearities.


\end{itemize}

\begin{figure}
  \centering
  \includegraphics[width=0.6\linewidth]{directions-aware_scheduling.eps}
  \caption{Sum rate as a function of SNR for different levels of EVM. In this example, 4 UEs are co-scheduled employing MRT precoding and sub-band scheduling with $M = 100$ antennas.}
  \label{fig:sum_rate_mrt}
\end{figure}


% ----------------------------------------------------------------%
%                       QUESTION 3                                %
% ----------------------------------------------------------------%
\noindent\colorbox{light-gray}{\begin{minipage}{7.0truein}
\begin{itemize}
\item[3.]{\bf Comment:} In commercial base stations, the nonlinear problem of power amplifier can be solved by digital pre-distortion (DPD), building compensation circuit and power back-off. Does this study have commercial value in practice?
\end{itemize}
\end{minipage}}

\begin{itemize}
\item[]{\bf Response:} Yes, in practical systems, managing nonlinear distortion to acceptable levels often involves designing appropriate digital predistorters (DPD). These predistorters compensate for nonlinear distortion and ensure sufficiently linear-like amplification of the transmitted signal to meet distortion requirements. However, with the advent of 5G wireless networks, channel bandwidth has increased significantly compared to previous generations. As a result, methods such as DPD become less practical because they require oversampling rates five to seven times higher than channel bandwidth\cite{mikko}. Even if DPD is used, their will be residual non-linearities; hence, it should be perceived as a way to reduce the distortion, not a way to remove it entirely.

To effectively address non-linear distortion, alternative solutions that do not rely on high oversampling are needed. Such approaches should aim to maintain low complexity and power consumption in multi-antenna transmitters. Additionally, while power back-off can help mitigate non-linear distortion, it comes at the cost of reduced performance.

Furthermore, the derived theorem in this paper provides a foundation for developing baseband algorithms that can predict and compensate for nonlinear distortion, as illustrated in the response to Comment 1. These algorithms can potentially serve as viable alternatives to traditional methods such as DPD, ensuring high performance while reducing complexity and energy consumption.

\end{itemize}




==> tikz/01-multiport_antenna_array.tex <==
\begin{figure}
\centering
\begin{circuitikz}
 %\draw (0,0) node[minimum height=3cm,minimum width=1.5cm,draw] {$\matZ_{\text{AT}}$};
\draw (0,0) -- (1.5,0) -- (1.5,3) -- (0,3) -- (0,0);
\node at (0.75,1.5) {$\matZ_{\text{AT}}$};

%terminals
\draw[{Circle[open]}-] (-0.75,0.2) -- (0,0.2); %port2 -
\draw[{Circle[open]}-] (-0.75,1) -- (0,1);       %port2 +
\draw[{Circle[open]}-] (-0.75,2) -- (0,2);       %port1 -
\draw[{Circle[open]}-] (-0.75,2.8) -- (0,2.8); %port1 +

%currents
\draw[-Stealth] (-0.55,1) -- (-0.1,1) node[midway,above]{$i_N$};
\draw[Stealth-] (-0.55,0.2) -- (-0.1,0.2);

\draw[-Stealth] (-0.55,2.8) -- (-0.1,2.8) node[midway,above]{$i_1$};
\draw[Stealth-] (-0.55,2) -- (-0.1,2);

%voltages
\node at (-0.75,2.4) (v1) {$v_1$};
\node at (-0.75,0.6) (v2) {$v_N$};

%signs
\node [above of=v1,node distance=0.25cm] {+};
\node [below of=v1,node distance=0.25cm] {--};

\node [above of=v2,node distance=0.25cm] {+};
\node [below of=v2,node distance=0.25cm] {--};

\end{circuitikz}
\caption{A system of $N$ antenna modeled by a linear $N$-port device.}
\label{fig:n_port_antenna}
\end{figure}






==> tikz/02-multiport_system_model.tex <==


\def\xt{-1}
\def\yt{4.5}
\def\ph{1.5}
\def\pd{3}

\begin{figure*}
\centering
\begin{circuitikz} [scale=1]
%\draw [help lines, dashed, xstep=0.5cm,ystep=0.5cm] (-1,-2) grid (17,6);

%%%%%%%%%%%%%%%%%%%%%%%%% Source Generation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%Port 1 
\draw (\xt,\yt-\ph) to[/tikz/circuitikz/bipoles/length=0.8cm, sV,v_=$v_{S,1} $] (\xt,\yt) ;  %Source 1

\draw (\xt,\yt) to[european,/tikz/circuitikz/bipoles/length=0.8cm,xshift=-0.2cm,R,
i>=$i_{T,1}$, l=$R$] (\xt+1.5+0.2,\yt); %Resistor 1
\draw (\xt,3) -- (\xt+1.5,\yt-\ph);

\def\ytt{\yt-\pd}



% Port 2 
\draw (\xt,\ytt-\ph) to[/tikz/circuitikz/bipoles/length=0.8cm, sV,v=$v_{s,N}$] (\xt,\ytt); %Source 2

\draw (-1,1.5) to[european,/tikz/circuitikz/bipoles/length=0.8cm,R, i>=$i_{T,N}$, l=$R$] (0.5,1.5); %Resistor 2
\draw (-1,0) -- (0.5,0);


%%%%%%%%%%%%%%%%%%%%%%%%% TX Impedance Matrix %%%%%%%%%%%%%%%%%%%%%%%%%%

\draw (1,-0.5) -- (2.5,-0.5) -- (2.5,5) -- (1,5) -- (1,-0.5);
\node at (1.75,2.25) {$\matZ_{\text{MT}}$};

%terminals
\draw[{Circle[open]}-] (0.5,4.5) -- (1,4.5);       %port1 +
\draw[{Circle[open]}-] (0.5,3)   -- (1,3);         %port1 -

\draw[{Circle[open]}-] (0.5,1.5) -- (1,1.5);       %port2 +
\draw[{Circle[open]}-] (0.5,0)   -- (1,0);         %port2 -

\draw[-{Circle[open]}] (2.5,4.5) -- (3,4.5);       %port3 +
\draw[-{Circle[open]}] (2.5,3)   -- (3,3);         %port3 -

\draw[-{Circle[open]}] (2.5,1.5) -- (3,1.5);       %port4 +
\draw[-{Circle[open]}] (2.5,0)   -- (3,0);         %port4 -

%voltages
\node at (0.5,3.75) (v1) {$v_{T,1}$};
\node at (0.5,0.75) (v2) {$v_{T,N}$};

%signs
\node [above of=v1,node distance=0.5cm] {+}; 
\node [below of=v1,node distance=0.5cm] {--};

\node [above of=v2,node distance=0.5cm] {+};
\node [below of=v2,node distance=0.5cm] {--};


%%%%%%%%%%%%%%%%%%%%%%% Z_T %%%%%%%%%%%%%%%%%%%


\draw (3.5,-0.5) -- (5,-0.5) -- (5,5) -- (3.5,5) -- (3.5,-0.5);
\node at (4.25,2.25) {$\matZ_{\text{AT}}$};

\draw (3,4.5) -- (3.5,4.5); 
\draw (3,3)   -- (3.5,3);

\draw (3,1.5) -- (3.5,1.5);
\draw (3,0)   -- (3.5,0); 

%currents
\draw[-Stealth] (3,4.5) -- (3.5,4.5) 
node[midway,above left = -2pt]{$i_{A,1}$}; %P1

\draw[-Stealth] (3,1.5) -- (3.5,1.5) node[midway,above left = -2.5pt]{$i_{A,N}$}; %PN

%voltages
\node at (3,3.75) (vA1) {$v_{A,1}$};
\node at (3,0.75) (vA2) {$v_{A,N}$};

%signs
\node [above of=vA1,node distance=0.5cm] {+}; 
\node [below of=vA1,node distance=0.5cm] {--};

\node [above of=vA2,node distance=0.5cm] {+};
\node [below of=vA2,node distance=0.5cm] {--};

%%%%%%%%%%%%%%%%%%%%%%% Z_R %%%%%%%%%%%%%%%%%%%


\draw (6.5,-0.5) -- (8,-0.5) -- (8,5) -- (6.5,5) -- (6.5,-0.5);
\node at (7.25,2.25) {$\matZ_{\text{AR}}$};

%Ports
\draw[-{Circle[open]}] (8,4.5) -- (8.5,4.5); 
\draw[-{Circle[open]}] (8,3)   -- (8.5,3);

\draw[-{Circle[open]}] (8,1.5) -- (8.5,1.5);
\draw[-{Circle[open]}] (8,0)   -- (8.5,0); 

%voltages
\node at (8.5,3.75) (vB1) {$v_{B,1}$};
\node at (8.5,0.75) (vB2) {$v_{B,N}$};

%signs
\node [above of=vB1,node distance=0.5cm] {+}; 
\node [below of=vB1,node distance=0.5cm] {--};

\node [above of=vB2,node distance=0.5cm] {+};
\node [below of=vB2,node distance=0.5cm] {--};




%%%%%%%%%%%%%%%%% Extrinsic Noise %%%%%%%%%%%%%%%


\draw (8.5,4.5) to[/tikz/circuitikz/bipoles/length=1.0cm, sV,v=$v_{E,1}$] (10,4.5);

\draw (8.5,3) -- (10,3);

\draw (8.5,1.5) to[/tikz/circuitikz/bipoles/length=1.0cm, sV,v=$v_{E,N}$] (10,1.5);

\draw (8.5,0) -- (10,0);

%%%%%%%%%%%%%%%%%%%%%%% Z_MR %%%%%%%%%%%%%%%%%%%

\draw (10.5,-0.5) -- (12,-0.5) -- (12,5) -- (10.5,5) -- (10.5,-0.5);
\node at (11.25,2.25) {$\matZ_{\text{MR}}$};

%Terminals (left)
\draw[{Circle[open]}-] (10,4.5) -- (10.5,4.5); 
\draw[{Circle[open]}-] (10,3)   -- (10.5,3);

\draw[{Circle[open]}-] (10,1.5) -- (10.5,1.5);
\draw[{Circle[open]}-] (10,0)   -- (10.5,0); 

%Terminals (right)
\draw[-{Circle[open]}] (12,4.5) -- (12.5,4.5); 
\draw[-{Circle[open]}] (12,3)   -- (12.5,3);

\draw[-{Circle[open]}] (12,1.5) -- (12.5,1.5);
\draw[-{Circle[open]}] (12,0)   -- (12.5,0); 



%voltages
\node at (12.5,3.75) (vR1) {$v_{R,1}$};
\node at (12.5,0.75) (vR2) {$v_{R,N}$};

%signs
\node [above of=vR1,node distance=0.5cm] {+}; 
\node [below of=vR1,node distance=0.5cm] {--};

\node [above of=vR2,node distance=0.5cm] {+};
\node [below of=vR2,node distance=0.5cm] {--};




%%%%%%%%%%%%%%%%%%%%%%% receive amplifier %%%%%%%%%%%%%%%%%%%

%Port 1
\draw (14.5,4.5) to[/tikz/circuitikz/bipoles/length=1.0cm, sV,v_=$v_{I,1}$] (12.5,4.5);

\draw (14.5,3) to[american,/tikz/circuitikz/bipoles/length=0.8cm,R, I=$i_{I,1}$] (14.5,4.5);

\draw (15.5,3) to[european,/tikz/circuitikz/bipoles/length=0.8cm,R, v=$v_{L,1}$, l=$R$] (15.5,4.5);

\draw (15.5,3) -- (12.5,3);
\draw (15.5,4.5) -- (14.5,4.5);


%Port N
\draw (14.5,1.5) to[/tikz/circuitikz/bipoles/length=1.0cm, sV,v_=$v_{I,N}$] (12.5,1.5);

\draw (14.5,0) to[american,/tikz/circuitikz/bipoles/length=0.8cm,R, I=$i_{I,N}$] (14.5,1.5);

\draw (15.5,0) to[european,/tikz/circuitikz/bipoles/length=0.8cm,R, v=$v_{L,N}$, l=$R$] (15.5,1.5);

\draw (15.5,0) -- (12.5,0);
\draw (15.5,1.5) -- (14.5,1.5);

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[dashed] (3,-0.75) -- (8.5,-0.75) -- (8.5,5.25) -- (3,5.25) -- (3,-0.75) ;
\node at (5.75,5.5) {$\matZ_{\text{A}}$};

\draw [decorate,decoration={brace, amplitude=10pt},
			xshift=0pt, yshift=0pt]
			(2.75,-1) -- (-1,-1)
			node[black,midway,yshift=-20pt]
				{transmitter's side};

\draw [decorate,decoration={brace, amplitude=10pt},
			xshift=0pt, yshift=0pt]
			(10,-1) -- (3,-1)
			node[black,midway,yshift=-20pt,text width=10cm,align=center]
				{mutial coupling among all transmitter's and receiver's antennas, and reception of extrinsic noise};
\draw [decorate,decoration={brace,amplitude=10pt},
			xshift=0pt, yshift=0pt]
			(16,-1) -- (10.25,-1)
			node[black,midway,yshift=-20pt, text width=5cm,align=center]
				{receiver's side with noisy receive amplifier};



\end{circuitikz}
\caption{Linear multiport model of a radio multi-antenna communication system.}
\label{fig:multiport_model}
\end{figure*}




%\draw (0,1.5) -- ++(0.5,0)
%to[american,open, v=$v_{T,1}$, o-o] ++(2,0) -- ++(0.5,0);

%\draw node[ocirc] (A) at (1.25,0) {-};
%\draw node[ocirc] (B) at (1.25,1.5) {+};
%\draw (B) to[open, v=$v_{T,1}$] (A);

==> tikz/03-equivalent_representation.tex <==
\tikzstyle{block} = [draw, fill=white, rectangle, 
    minimum height=3em, minimum width=4em]
\tikzstyle{sum} = [draw, fill=white, circle, node distance=1cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\begin{figure}
\centering
\subfloat[Nonlinear system]{%
  \begin{tikzpicture}[auto, node distance=2cm,>=latex',
amp/.style = {regular polygon, regular polygon sides=3,
              draw, fill=white, text width=1.5em,
              inner sep=1mm, outer sep=0mm,
              shape border rotate=-90}]
              
    \node [input, name=input] {};
    \node [amp, right of=input,
            node distance=2cm] (system) {PA};
    \node [output, right of=system,
            node distance=2cm] (output) {};
    
    \draw [->] (input) -- node[name=x] {$x_b[n]$} (system);    
    \draw [->] (system) -- node[name=u] {$y_b[n]$} (output);
\end{tikzpicture}
}
\vspace{0.5cm}
\subfloat[Equivalent linear system]{%
  \begin{tikzpicture}[auto, node distance=1cm,>=latex']
              
    \node [input, name=input] {};
    \node [block, right of=input,
            node distance=2cm] (system) {$\tilde{c}_b[n]$};
    \node [sum, right of=system,
            node distance=2cm] (sum) {+};
    \node [output, right of=sum,
            node distance=1.2cm] (output) {};
    \node [below of=sum,
            node distance=1cm] (distortion) {};
    
    \draw [->] (input) -- node[name=x] {$x_b[n]$} (system);    
    \draw [->] (system) -- node[name=u] {$u_b[n]$} (sum);
    \draw [->] (sum) -- node [name=y] {$y_b[n]$}(output);
    \draw [->] (distortion) -- node [name=d] {$d_b[n]$}(sum);

\end{tikzpicture}
}
\caption{Equivalent representations of an OFDM signal.}

\end{figure}
